Viscosity in water from first-principles and deep-neural-network simulations

We report on an extensive study of the viscosity of liquid water at near-ambient conditions, performed within the Green-Kubo theory of linear response and equilibrium ab initio molecular dynamics (AIMD), based on density-functional theory (DFT). In order to cope with the long simulation times necessary to achieve an acceptable statistical accuracy, our ab initio approach is enhanced with deep-neural-network potentials (NNP). This approach is first validated against AIMD results, obtained by using the Perdew-Burke-Ernzerhof (PBE) exchange-correlation functional and paying careful attention to crucial, yet often overlooked, aspects of the statistical data analysis. Then, we train a second NNP to a dataset generated from the Strongly Constrained and Appropriately Normed (SCAN) functional. Once the error resulting from the imperfect prediction of the melting line is offset by referring the simulated temperature to the theoretical melting one, our SCAN predictions of the shear viscosity of water are in very good agreement with experiments.

==> table1.tex <==
\begin{table}[ht]
\caption{
Viscosity of water [cP] computed from AIMD or DPMD performed at two different temperatures using the PBE XC functional.
} 
\centering
\begin{tabular}{lcc}
\textrm{}&
\textrm{T $= 454$ K}&
\textrm{T $= 600$ K} \\
\hline

\text{AIMD} &  0.383 $\pm$ 0.023 & 0.178 $\pm$ 0.005 \\
\text{DPMD}  &  0.402 $\pm$ 0.005 & 0.184 $\pm$ 0.001  \\

\end{tabular}
\end{table}

==> table2.tex <==
\begin{table}[ht]
\caption{
Shear viscosity [cP] computed for water at different temperatures with PBE-NNP force field and using simulation boxes of different size. 
}
\centering
\begin{tabular}{lccc}
&
\multicolumn{3}{c}{size (number of molecules)}\\
\textrm{T [K]}&
64&
512&
4096 \\
\hline
 454  & 0.402 $\pm$ 0.005  & 0.402 $\pm$ 0.005 & 0.417 $\pm$ 0.007  \\
600 & 0.184 $\pm$ 0.001  &
        0.186 $\pm$ 0.002 &
        0.186 $\pm$ 0.002 \\
\end{tabular}
\end{table}
